Are We Building on the Rock? On the Importance of Data Preprocessing for Code Summarization

Code summarization, the task of generating useful comments given the code, has long been of interest. Most of the existing code summarization models are trained and validated on widely-used code comment benchmark datasets. However, little is known about the quality of the benchmark datasets built from real-world projects. Are the benchmark datasets as good as expected? To bridge the gap, we conduct a systematic research to assess and improve the quality of four benchmark datasets widely used for code summarization tasks. First, we propose an automated code-comment cleaning tool that can accurately detect noisy data caused by inappropriate data preprocessing operations from existing benchmark datasets. Then, we apply the tool to further assess the data quality of the four benchmark datasets, based on the detected noises. Finally, we conduct comparative experiments to investigate the impact of noisy data on the performance of code summarization models. The results show that these data preprocessing noises widely exist in all four benchmark datasets, and removing these noisy data leads to a significant improvement on the performance of code summarization. We believe that the findings and insights will enable a better understanding of data quality in code summarization tasks, and pave the way for relevant research and practice.

==> bak/3.CleanTool-w-sem.tex <==
\section{The Taxonomy of Noisy Data}

To develop a taxonomy of noisy data for code summarization tasks, we employ an \textit{open card sort} \cite{DBLP:journals/es/RuggM05} process by involving nine  participants. 
{Participants include two PhD students, four master students, and three senior researchers. 
All of them are fluent English speakers, and have done either intensive research work with software development or have been actively contributing to open-source projects.}
The sorting process is conducted in multiple rounds. In the first round,
all participants label the same sample of benchmark data, with an intensive discussion session to achieve conceptual coherence about noisy categories. The average Cohen’s Kappa is 0.86.
Then, a shared pool of categories is utilized and carefully maintained, and
each participant could select existing categories from and/or add new category names into the shared pool. The sorting process ends when there is no new category added for two consecutive rounds. In total, we conducted 10 rounds and labeled 1600 pairs of code summary (400 pairs for each four benchmark datasets).
{Among them, we annotated XXX syntactic noises, XXX non-summary comments, and XXX summary comments.} \lin{@fangwen}\lin{updated @Ge}
The detail annotation results are shown in Table \ref{table:rq2_dataset}. {Next, we introduce 11 categories of syntactic noise and one category (non-summary) of semantic noise, as well as and their examples in the following.} 

% \jie{here, we may need to explicit state which categories are syntactic noise and which categories are semantic noise.}\lin{updated}


%  \begin{figure*}[]
% \centering
%  \includegraphics[width=\textwidth,height=21.5cm]{fig/taxonomy-tab.pdf}
%  %\vspace{-0.3cm}
%  \label{tab:tax-tmp}
%  \end{figure*}


\input{sec/taxonomy-2}



\section{The Code-Summary Cleaning Tool}

 

In this section, we introduce our automated data cleaning tool for code summarization datasets. As shown in Figure \ref{fig:overview}, the tool consists of two subsequent cleaners, a rule-based syntactic cleaner and a model-based semantic cleaner. First, the rule-based syntactic cleaner is used for removing syntactic noises, and then the model-based semantic cleaner is used for classifying non-summary and summary comments from the rest (Note that, we refer to semantic noises as non-summary comments and refer to normal comments as summary comments in this study).\lin{updated @Ge} 
%The origin code-summary pairs in benchmark datasets are firstly cleaned by the rule-based cleaner, where a set of heuristic rules are applied to detect the existence of invalid syntax.  Next, we further filter semantic noise based on our model-based cleaner, which is trained on an external dataset.
In the following, we first elaborate on the design of the two subsequent cleaners, and then report the effectiveness evaluation of the tool.

\subsection{The Syntactic Cleaner}

%According to common practice guidance, e.g., Javadoc guidance \cite{}, 
%http://www.oracle.com/technetwork/articles/java/index-137868.html
%the first sentences of the code comments typically describe the code functionalities. 
%Therefore, nearly all the existing researches extract the first sentences of the code comments as the target summaries. 

%Since raw data can hardly be directly used for code summarization tasks, nearly all the existing benchmark datasets are constructed under multiple preprocessing operations, e.g., using `newline' as the delimiter to collect the first sentence in the comments \cite{leclair2019neural}.
%\jie{not only the preprocessing, but also the data itself, cause the noise in the data. i think this current statement might be misleading.}
%However, we have a concern that about how well are these preprocessing operations performed in constructing benchmark datasets. 
%To address the above concern, we develop a syntactic cleaner with a set of heuristic rules that can precisely identify syntactic noises.

%\subsubsection{Taxonomy of syntactic noises.} 


%We introduce the taxonomy of syntactic noises and their examples in Table XXX.
To automatically detect each category of syntactic noises in the taxonomy, we develop a syntactic cleaner with a set of heuristic rules.
The heuristic rules comply with three criteria: (1) Any rule should define a unique and
specific construction category; (2) The rules should limit the preclusion of valid data within an acceptable range \jie{the reviewers might argue what is the `acceptable range?'}\lin{I follow previous study when state this, our inspection shows all above 90\% F1 score, any idea how can we update here @junjie}\jie{i am not sure}; and (3) Any rule is not a subrule of other rules in the set. 
Table \ref{tab:taxonomy} demonstrates the syntax feature of heuristic rules and our actions.

% Algorithm 1 illustrates the details of the syntactic cleaner detecting and correcting Partial sentence and Verbose sentences. Initially, we set the first sentence of raw comment $FS$ with an empty string and define three regex.
% Then, we split the input raw comment $RC$ into a comment list $L$ using newline character (5-th lines). We loop through each comment line $l$ in the comment List $L$ until the first sentence is extracted (6-th to 17-th lines).  Specifically, at each loop time, we first remove the comment tags such as `*' at start of the comment line $l$ by using regex1 (12-th lines). We then use the regex2 to determine whether the current comment line $l$ contains a complete sentence. If not, we splice the current comment line $l$ to the end of the existing first sentence $FS$ (13-th to 17-th lines). If the existing $FS$ is not empty, we use regex3 to determine whether the current comment line l starts with an uppercase letter or special tags, and if so, we take the existing $FS$ string as the first sentence and break the loop (8-th to 9-th lines). Finally, we determine the noise category of the benchmark comment $BC$ by comparing its length with the extracted first sentence $FS$ (18-th to 22-th lines).
%\input{table/alg}


 \begin{figure}[t]
\centering
 \includegraphics[width=0.9\columnwidth]{fig/alg.pdf}
 %\vspace{-0.3cm}
 \caption{If-else rules of collecting the first sentence in the raw comments for partial and verbose sentence noises.}
 \label{fig:3-flow}
 \end{figure}


We develop heuristic rules for detecting each category of syntactic noises. Taking the partial and verbose sentence category as an example, first, we carefully identify their syntax features from part of the manually annotated noises. Then, we design a set of if-else rules to collect the correct first sentence from the raw data, and test their correctness on the rest of the manually annotated noises. \lin{updated @Ge}
(Note that, the raw data refers to the source data that has not been processed for use, and the origin data refers to the processed raw data by benchmark datasets). 
% \jie{what is the raw data}\lin{updated}. 
Second, by comparing the first sentence we extracted with the data provided in the benchmark dataset, we can determine the verbose or partial sentence category.
Figure \ref{fig:3-flow} 
% \jie{the title of this figure is not good. the figure is vague}\lin{updated}
illustrates the if-else rules of collecting the first sentence in the raw comments for partial and verbose sentence noises. The key idea is to sequentially determine whether each comment line in a raw comment contains a complete sentence, and if so, return the first complete sentence; if not, save the content of the line and continue to determine the next line. \lin{@updated @junjie}
% Initially, we set the first sentence of raw comment $FS$ with an empty string. Then, we extract the $FS$ by iterating over each comment line $L$ in a raw comment. The entire loop body consists of three conditional statements. 
% \jie{it is a little weird the third statement is first mentioned.}\lin{@fangwen}
% The third conditional statement determines whether the current $L$ contains at least one split sentence. If $L$ contains no sentences, then we splice the entire $L$ to the end of the current $FS$; else, we splice the first split sentence in $L$ to the end of the current $FS$ and return the $FS$. 
% Since many developers do not use the standard terminators such as period to indicate an ending sentence when writing comments (see the example of Verbose sentence in Table \ref{tab:taxonomy}), we utilize the first and second conditional statements to judge whether the sentence ends. Precisely, if $FS$ is not empty, we determine whether the current comment line $L$ starts with an uppercase letter. If $L$ is capitalized, we return the $FS$; if not, we proceed to the third conditional statement.

Details of the heuristic rules for other categories can be found on our website \cite{website}. 

\input{table/RQ1_v3}
 




%Note that we focus on syntactic noises on summaries and code in the syntactic cleaner, and leave the semantic analysis to the semantic cleaner.


\subsection{The Semantic Cleaner}
%\mfw{Developers may write comments for other intentions, such as copyright and to-do, instead of describing the core functionalities of the code. For example, the hint message: "not in use" and the auto-generated message: "Description of the Method", which are semantically unrelated to the corresponding code, appear XXX and XXX times in {\funcom} dataset, respectively. We argue that such comments would mislead the model to focus on learning features that impair the generalization performance of itself, especially when these comments widely exist in datasets. Unfortunately, most researchers ignore to perform semantic analysis of comments when constructing the benchmark datasets, let alone cleaning noises from these datasets at the semantic level. In this work, we define the pairs whose comments are semantically unrelated to the corresponding code as semantic noises. To address the above concern, we introduce a model-based semantic cleaner trained on an external dataset to further refine the benchmark datasets by precisely filtering semantic noises.}

%Some existing studies are interested in the comment classification task and have provided high-quality labeled datasets. To simplify our data annotation work, we build our semantic cleaner based on Chen et al.'s dataset \cite{DBLP:journals/tosem/ChenXHLL21}. Chen \textit{et al}. have 

\lin{TBD: add rationale of using external data? @wangsong what do you think}
We utilize a manual-inspected external data provided by Chen et al.~\cite{DBLP:journals/tosem/ChenXHLL21} to train the semantic noise classifier. They classified comments into six categories: ``what'', ``why'', ``how-to-use'', ``how-it-is-done'', ``property'', and ``others''.  Following their work, we consider the first five categories as summary, and the ``others'' as non-summary noises. 

\textbf{GBDT Model.}
To classify non-summary noises, we employ the Gradient Boosting Decision Tree (GBDT) \cite{DBLP:conf/nips/KeMFWCMYL17} as our classification model.
% , which has been proven to be effective in comment classification tasks \cite{DBLP:conf/iwpc/SteidlHJ13, DBLP:journals/ese/PascarellaBB19, DBLP:journals/tosem/ChenXHLL21}. \lin{add cite asap @Fangwen}
%In this work, we employ the Gradient Boosting Decision Tree (GBDT) \cite{} as the semantic cleaner. GBDT is a widely-used machine learning model, and has been proven to be effective in comment classification in software engineering \cite{}. 
\jie{do we need such details of the model. it is a commonly used machine learning model. also i think using the `log-likelihood loss function' is a common practice.}\lin{TBD}
The GBDT is an ensemble model consisting of $k$ Decision Trees, and the latter algorithm has been proven to be effective in comment classification tasks \cite{DBLP:conf/iwpc/SteidlHJ13, DBLP:journals/ese/PascarellaBB19, DBLP:journals/tosem/ChenXHLL21}. \mfw{updated @Ge}
It can be formulated as:
\[\hat{y}_i=\sum\limits_{k=1}^K{f_k(x_i)},f_k\in F\]
where $f_k(x_i)$ is the $k-$th decision tree, $F$ is a functional space composed of all trees. It is trained in sequence, and each base model is added to correct the error produced by its previous tree models. For each step, the samples misclassified by previous models are more likely to be selected as the train data, producing more accurate prediction performance. We use the log-likelihood loss function to optimize the model:
\[L=\log(1+\exp(-y\hat{y}_i)\]
where $y$ is the ground-truth label, $\hat{y}_i$ is the predicted probability.

\input{table/RQ2_feature}

\textbf{Features.} 
% To enhance features and improve model performance, we consider three categories of features: textual features, statistical features, and syntactic features. For textual features, after tokenization of the comments, we extract tf-idf \cite{} vector of each word, which could determine the mathematical significance of words in comments. 
Based on our observation of the comment data, we find that non-summary data has statistical characteristics and content patterns that can be used to distinguish it from summary data. Thus, we define two categories features, which are statistical features and content features, as the input of the GBDT model.
% As shown in table \ref{tab:rq2_feature}, we consider two categories features, statistical features and content features, to train the GBDT model. 
\begin{figure*}[htpb]
\centering
\includegraphics[width=1.7\columnwidth]{fig/pie.pdf}
%\vspace{-0.3cm}
\caption{Percentage of syntactic (SYN) and semantic (SEM) noise in terms of removal and update.\lin{add overall}}
\label{fig:rq1-pie}
\end{figure*}

Table \ref{tab:rq2_feature} illustrates the detail information of these features.
For statistical features, after tokenization of the comment data, we extract TF-IDF \cite{DBLP:conf/sigir/SaltonY73} vector of each word, which could measure the mathematical significance of words in comments. This technique is a conventional feature extraction approach for the natural language text analysis in the software engineering literature \cite{behl2014bug}. We also extract the number of words and unique words, and calculate the percentage of punctuation and digits in comments.
For content features, we determine whether comments contain keywords such as ``todo", ``deprecate", ``copyright", ``FIXME:", and whether they contain code snippets or mathematical formulas. Such features are also used in prior software engineering literature \cite{DBLP:conf/iwpc/SteidlHJ13, DBLP:journals/ese/PascarellaBB19}.


\textbf{SMOTE.} The classification of summary and non-summary from the training 
%\jie{not from benchmark data? should be the training data?}
data is imbalanced in that the summary data are much more than the non-summary data. To alleviate the imbalance problem, we employ the synthetic minority over-sampling technique (SMOTE) \cite{DBLP:journals/jair/ChawlaBHK02}, which can avoid the over-fitting problem by generating new instances with the help of interpolation between the positive instances that lie together.



\subsection{Effectiveness Evaluation}
In this section, we evaluate the effectiveness our syntactic cleaner and semantic cleaner.
%To evaluate how effective is our code-summary cleaner in detecting syntactic and semantic noises, we perform an experiment on XXX manually-annotated data, and report the results in this section. 


\subsubsection{Data Preparation.}
As introduced in Section 3.1, we labeled 11 categories of syntactic noises from 1600 code-summary pairs sampled from the four datasets. 
Based on the data that are not labeled as syntactic noises, we further manually annotate them into summary and non-summary data. We use these manually annotated data to evaluate the performance of our cleaner. 
Table \ref{table:rq2_dataset} shows the detail. 
For syntactic cleaner, We build the heuristic rules based on observing the 80\% of the annotated syntactic noises, and evaluate on the rest 20\%. 
For semantic cleaner, we utilize the external dataset provided by Chen et al. \cite{DBLP:journals/tosem/ChenXHLL21} to train our model, and test the model on the summary and non-summary data that we manually  annotated. \lin{updated @Ge} 
%We aggregate the ``what'', ``why'', ``how-it-is-done'',``how-to-use'', and ``property'' labeled data as our summary data, and use the ``others'' as non-summary data.
%\jie{kind of duplicate with the statement in sec 4.2. }\lin{updated}




%\mfw{The effectiveness evaluation involves three types of datasets, including: (1) Manually annotated dataset \textit{SYN-manual}. The \textit{SYN-manual} dataset is first used to develop the taxonomy of syntactic noises. Then, we design the heuristic rules by observing 80\% of the labeled data in the dataset. Finally, we evaluate the performance of the syntactic cleaner on the remaining labeled data. (2) External dataset \textit{SEM-external}. The \textit{SEM-external} dataset is used to train the model-based semantic cleaner. (3) Manually annotated dataset \textit{SEM-manual}. The \textit{SEM-manual} dataset is used to validate the effectiveness of our semantic cleaner.}




% \textbf{SYN-manual dataset.}
% We randomly sample 1600 code-summary pairs (400 for each benchmark dataset) as 
% to build the \textit{SYN-manual} dataset. We recruit XXX participants to label the data by employing an open card sort process, as we mentioned in section 3.1. For each sample code-summary pair, we label ground-truth data from three aspects: (1) label code data with code-level syntactic noise categories, (2) label summary data with summary-level syntactic noise categories, (3) correct the code or summary data belonging to the updated noises. After the labeling process, we shuffle the dataset and use the first 80\% for building the heuristic rules, the rest 20\% for evaluating the performance of the syntactic cleaner in detecting and correcting noises.

% \textbf{SEM-external dataset.}
% We use an external dataset proposed by Chen et al. \cite{} to train our semantic cleaner. The dataset contains 20,000 code comments which are classified into six intention categories including "what", "why", "how-to-use", "how-it-is-done", "property", and "others". We take "others" comments as \textit{non-summary}, and the remaining categories of comments as \textit{summary}.



%technique, named Synthetic Minority Over-sampling Technique (SMOTE) \cite{}, which SMOTE is an oversampling technique where the synthetic samples are generated for the minority class. SMOTE focuses on the feature space to generate new instances with the help of interpolation between the positive instances that lie together. Compare to the arbitrary bootstrap sampling strategy \cite{}, this technique is able to generate synthetic instances rather than replicate minority class instances; therefore, it can avoid the over-fitting problem.


% \textbf{SEM-manual dataset.}
% To validate the effectiveness of our semantic cleaner, we also randomly sample 400 code-comment pairs from each benchmark dataset as the validation set. 
% We manually label each sampled data with summary and non-summary. To guarantee the correctness of the labeling results, we built an inspection team, which consisted of four Ph.D. candidates. All of them are fluent English speakers, and have done either intensive research work with software development or have been actively contributing to open-source projects. We divided the team into two groups. The labeled results from the Ph.D. candidates were reviewed by others. When a labeled result received different opinions, we hosted a discussion with all team members to decide through voting. The average Cohen’s Kappa is 0.72.

\subsubsection{Experimental setup}
We implement the model-based semantic cleaner using scikit-learn \cite{scikitlearn} which is an open-source data analysis and machine learning library. We train the GBDT model with log-likelihood loss function. 
{For the} hyper-parameters,
we use greedy search as the parameter tuning  method to
obtain the best performance.
{After the parameter tuning, we set the \textit{learning\_rate}=0.01, \textit{n\_estimators}=100, \textit{subsample}=1, and \textit{min\_samples\_leaf}=2.}

\subsubsection{Evaluation Metrics.}
% For syntactic noises detection, we use Micro-Precision, Micro-Recall, and Micro-F1 metrics \cite{}, which are commonly used in multiple classification tasks. These three metrics measure the precision, recall, and f1 of the aggregated contributions of all syntactic noise categories, respectively. We utilize Accuracy to evaluate the performance of syntactic noises correction\lin{add one sentence description of how calculate accuracy or cite something}. For semantic noises classification, we use the conventional classification metrics: Precision, Recall, and F1 \cite{}.

We use three commonly-used metrics to evaluate the performance of our cleaning tool, i.e., \textit{Precision}, \textit{Recall}, and \textit{F1}. (1) \textit{Precision} refers to the ratio of correct predictions to the total number of predictions; (2) \textit{Recall} refers to the ratio of correct predictions to the total number of samples in the golden test set; and (3) \textit{F1} is the harmonic mean of precision and recall. 


% When comparing the performances, we care more about F1 since it is balanced for evaluation. Note that the correction XXX.

\input{table/RQ2_dataset_v4}
\subsubsection{Results}

%\input{table/distilled-size}

%\input{table/syn-perf} 


%\input{table/sem-perf} 



Table \ref{table:rq2_dataset} demonstrates the performance of our two subsequent cleaners in terms of noisy data detection. We can see that, the syntactic cleaner can precisely detect syntactic noises on the four benchmark datasets. The Macro F1 scores are ranging from 97.61\% to 96.49\%, and 96.99\% on average, which is highly satisfactory \jie{highly satisfactory might not a good expression}\lin{@wangsong any suggestions?}.
%The accuracy of syntactic noise correction are ranging from 92.06\% to 95.18\%, which is also highly satisfactory. 
For semantic cleaner, the F1 scores of non-summary classification are ranging from 86.67\% to 92.86\%, and 91.74\% on average. The results show that, the semantic cleaner can also achieve a highly satisfactory performance on filtering non-summary noises.
In summary, Our code-summary cleaner can precisely filter noisy data syntactically and semantically, with all the F1 scores of over 90\%, {which help build a high-quality dataset for the follow-up code comment summary.}
%I think we should add a sentence like that.  }


% \noindent
% \begin{boxedminipage}[t]{\columnwidth}
% \jie{i think it isn't necessary to treat this as a separate finding. this is not a finding. }
% \textbf{Finding 1}:   
% \end{boxedminipage}

==> bak/3.CleanTool-w-tax.tex <==
\section{The Code-Summary Cleaning Tool}

In this section, we introduce our automated data
cleaning tool for code summarization datasets, mainly to filter out
code-summary pairs with syntactic or semantic noises. The tool consists of two subsequent cleaners, a rule-based syntactic cleaner and a
model-based semantic cleaner. 
An overview of the tool is shown in Figure \ref{fig:overview}.
The origin code-summary pairs in benchmark datasets are firstly cleaned
by the rule-based cleaner, where a set of heuristic rules are applied to detect the
existence of invalid syntax. 
Next, we further filter semantic noise based on our model-based cleaner, which is trained on an external dataset.
In the following, we first elaborate on the design of the two subsequent cleaners, and then report the effectiveness evaluation of the tool.

\subsection{The Syntactic Cleaner}


%According to common practice guidance, e.g., Javadoc guidance \cite{}, 
%http://www.oracle.com/technetwork/articles/java/index-137868.html
%the first sentences of the code comments typically describe the code functionalities. 
%Therefore, nearly all the existing researches extract the first sentences of the code comments as the target summaries. 

Since raw data can hardly be directly used for code summarization tasks, nearly all the existing benchmark datasets are constructed under multiple preprocessing operations, e.g., using `newline' as the delimiter to collect the first sentence in the comments \cite{leclair2019neural}.
\jie{not only the preprocessing, but also the data itself, cause the noise in the data. i think this current statement might be misleading.}
However, we have a concern that about how well are these preprocessing operations performed in constructing benchmark datasets. 
To address the above concern, we develop a syntactic cleaner with a set of heuristic rules that can precisely identify syntactic noises.

%\subsubsection{Taxonomy of syntactic noises.} 

To develop a taxonomy of syntactic noises for both code data and summary data, we employ an \textit{open card sort} \cite{DBLP:journals/es/RuggM05} process by involving XXX participants. \lin{add demographical profiles@fangwen}
The sorting process is conducted in multiple rounds. In the first round,
all participants label the same sample of benchmark data, with an intensive discussion session to achieve conceptual coherence about noisy categories. The average Cohen’s Kappa is 0.86.
Then, a shared pool of categories is utilized and carefully maintained, and
each participant could select existing categories from and/or add new category names into the shared pool. The sorting process ends when there is no new category added for two consecutive rounds. In total, we conducted XX rounds and labeled 1600 pairs of code summary (400 pairs for each four benchmark datasets). The detail annotation results are shown in XXX.
%We introduce the taxonomy of syntactic noises and their examples in Table XXX.

To automatically detect each category of syntactic noises in the taxonomy, we develop a syntactic cleaner with a set of heuristic rules.
The heuristic rules comply with three criteria: (1) Any rule should define a unique and
specific construction category; (2) The rules should limit the preclusion of valid data within an acceptable range; and (3) Any rule is not a subrule of other rules in the set.
Limited by the space, the details of the heuristic rules can be found on our website \cite{}. 

Table \ref{tab:taxonomy} demonstrates the taxonomy of syntactical noises, syntax feature of heuristic rules, real-world examples, and our corrections. 




%Note that we focus on syntactic noises on summaries and code in the syntactic cleaner, and leave the semantic analysis to the semantic cleaner.


\subsection{The Semantic Cleaner}
%\mfw{Developers may write comments for other intentions, such as copyright and to-do, instead of describing the core functionalities of the code. For example, the hint message: "not in use" and the auto-generated message: "Description of the Method", which are semantically unrelated to the corresponding code, appear XXX and XXX times in {\funcom} dataset, respectively. We argue that such comments would mislead the model to focus on learning features that impair the generalization performance of itself, especially when these comments widely exist in datasets. Unfortunately, most researchers ignore to perform semantic analysis of comments when constructing the benchmark datasets, let alone cleaning noises from these datasets at the semantic level. In this work, we define the pairs whose comments are semantically unrelated to the corresponding code as semantic noises. To address the above concern, we introduce a model-based semantic cleaner trained on an external dataset to further refine the benchmark datasets by precisely filtering semantic noises.}


In this work, we build our semantic cleaner based on Chen et al.'s dataset \cite{DBLP:journals/tosem/ChenXHLL21}. 
Chen \textit{et al}. have classified comments into six categories: ``what'', ``why'', ``how-to-use'', ``how-it-is-done'', ``property'', and ``others''.  Following their work, we consider the first five categories as summary, and the ``others'' as non-summary noises. 

\textbf{GBDT Model.}
To classify non-summary noises, we employ the Gradient Boosting Decision Tree (GBDT) \cite{} as our classification model, which has been proven to be effective in comment classification tasks \cite{}.
%In this work, we employ the Gradient Boosting Decision Tree (GBDT) \cite{} as the semantic cleaner. GBDT is a widely-used machine learning model, and has been proven to be effective in comment classification in software engineering \cite{}. 
The GBDT is an ensemble model consisting of $k$ decision trees:
\[\hat{y}_i=\sum\limits_{k=1}^K{f_k(x_i)},f_k\in F\]
where $f_k(x_i)$ is the $k-$th decision tree, $F$ is a functional space composed of all trees. It is trained in sequence, and each base model is added to correct the error produced by its previous tree models. For each step, the samples misclassified by previous models are more likely to be selected as the train data, producing more accurate prediction performance. We use the log-likelihood loss function to optimize the model:
\[L=\log(1+\exp(-y\hat{y}_i)\]
where $y$ is the ground-truth label, $\hat{y}_i$ is the predicted probability.

\input{table/RQ2_feature}

\textbf{Features.} 
% To enhance features and improve model performance, we consider three categories of features: textual features, statistical features, and syntactic features. For textual features, after tokenization of the comments, we extract tf-idf \cite{} vector of each word, which could determine the mathematical significance of words in comments. 
{Based on our observation of the external dataset, we find that non-summary data has statistical characteristics and content patterns that can be used to distinguish it from summary data. Thus, we define two categories features, which are statistical features and content features, as the input of the GBDT model.}
% As shown in table \ref{tab:rq2_feature}, we consider two categories features, statistical features and content features, to train the GBDT model. 
Table \ref{tab:rq2_feature} illustrates the detail information of these features.
For statistical features, after tokenization of the comment data, we extract TF-IDF \cite{} vector of each word, which could measure the mathematical significance of words in comments. This technique is a conventional feature extraction approach for the natural language text analysis in the software engineering literature \cite{}. We also extract the number of words and unique words, and calculate the percentage of punctuation and digits in comments.
For content features, we determine whether comments contain keywords such as ``todo", ``deprecate", ``copyright", ``FIXME:", and whether they contain code snippets or mathematical formulas. Such features are also used in prior software engineering literature \cite{}.

\textbf{SMOTE.} The classification of summary and non-summary from benchmark data is imbalanced in that the summary data are much more than the non-summary data. To alleviate the imbalance problem, we employ the synthetic minority over-sampling technique (SMOTE) \cite{}, which can avoid the over-fitting problem by generating new instances with the help of interpolation between the positive instances that lie together.


\subsection{Effectiveness Evaluation}
In this section, we evaluate the effectiveness our syntactic cleaner and semantic cleaner by manual inspection.
%To evaluate how effective is our code-summary cleaner in detecting syntactic and semantic noises, we perform an experiment on XXX manually-annotated data, and report the results in this section. 
\input{table/RQ2_dataset_v4}
\subsubsection{Data Preparation.}
As introduced in section 3.1, we labeled 11 categories of syntactic noises from 1600 code-summary pairs sampled from the four datasets. Based on the data that are not labeled as syntactic noises, we further manually annotate them into summary and non-summary data. We use these manually annotated data to evaluate the performance of our cleaner. 
Table XX shows the detail. 
For syntactic cleaner, We build the heuristic rules based on observing the 80\% of our annotated data, and evaluate on the rest 20\%. 
For semantic cleaner, we utilize the external dataset provided by Chen et al. \cite{DBLP:journals/tosem/ChenXHLL21} to train our model. We aggregate the ``what'', ``why'', ``how-it-is-done'',``how-to-use'', and ``property'' labeled data as our summary data, and use the ``others'' as non-summary data. We test the model on our manual annotated data.





%\mfw{The effectiveness evaluation involves three types of datasets, including: (1) Manually annotated dataset \textit{SYN-manual}. The \textit{SYN-manual} dataset is first used to develop the taxonomy of syntactic noises. Then, we design the heuristic rules by observing 80\% of the labeled data in the dataset. Finally, we evaluate the performance of the syntactic cleaner on the remaining labeled data. (2) External dataset \textit{SEM-external}. The \textit{SEM-external} dataset is used to train the model-based semantic cleaner. (3) Manually annotated dataset \textit{SEM-manual}. The \textit{SEM-manual} dataset is used to validate the effectiveness of our semantic cleaner.}




% \textbf{SYN-manual dataset.}
% We randomly sample 1600 code-summary pairs (400 for each benchmark dataset) as 
% to build the \textit{SYN-manual} dataset. We recruit XXX participants to label the data by employing an open card sort process, as we mentioned in section 3.1. For each sample code-summary pair, we label ground-truth data from three aspects: (1) label code data with code-level syntactic noise categories, (2) label summary data with summary-level syntactic noise categories, (3) correct the code or summary data belonging to the updated noises. After the labeling process, we shuffle the dataset and use the first 80\% for building the heuristic rules, the rest 20\% for evaluating the performance of the syntactic cleaner in detecting and correcting noises.

% \textbf{SEM-external dataset.}
% We use an external dataset proposed by Chen et al. \cite{} to train our semantic cleaner. The dataset contains 20,000 code comments which are classified into six intention categories including "what", "why", "how-to-use", "how-it-is-done", "property", and "others". We take "others" comments as \textit{non-summary}, and the remaining categories of comments as \textit{summary}.



%technique, named Synthetic Minority Over-sampling Technique (SMOTE) \cite{}, which SMOTE is an oversampling technique where the synthetic samples are generated for the minority class. SMOTE focuses on the feature space to generate new instances with the help of interpolation between the positive instances that lie together. Compare to the arbitrary bootstrap sampling strategy \cite{}, this technique is able to generate synthetic instances rather than replicate minority class instances; therefore, it can avoid the over-fitting problem.


% \textbf{SEM-manual dataset.}
% To validate the effectiveness of our semantic cleaner, we also randomly sample 400 code-comment pairs from each benchmark dataset as the validation set. 
% We manually label each sampled data with summary and non-summary. To guarantee the correctness of the labeling results, we built an inspection team, which consisted of four Ph.D. candidates. All of them are fluent English speakers, and have done either intensive research work with software development or have been actively contributing to open-source projects. We divided the team into two groups. The labeled results from the Ph.D. candidates were reviewed by others. When a labeled result received different opinions, we hosted a discussion with all team members to decide through voting. The average Cohen’s Kappa is 0.72.

\subsubsection{Experimental setup}
We implement the model-based semantic cleaner using scikit-learn \cite{} which is an open-source data analysis and machine learning library. We train the GBDT model with \textit{learning\_rate}=0.01. We set the \textit{n\_estimators}=100, \textit{subsample}=1, and \textit{min\_samples\_leaf}=2. For these hyper-parameters,
we use greedy search as the parameter selection method to
obtain the best performance.

\subsubsection{Evaluation Metrics.}
% For syntactic noises detection, we use Micro-Precision, Micro-Recall, and Micro-F1 metrics \cite{}, which are commonly used in multiple classification tasks. These three metrics measure the precision, recall, and f1 of the aggregated contributions of all syntactic noise categories, respectively. We utilize Accuracy to evaluate the performance of syntactic noises correction\lin{add one sentence description of how calculate accuracy or cite something}. For semantic noises classification, we use the conventional classification metrics: Precision, Recall, and F1 \cite{}.

We use three commonly-used metrics to evaluate the performance of our cleaning tool, i.e., \textit{Precision}, \textit{Recall}, and \textit{F1}. (1) \textit{Precision} refers to the ratio of the number of correct predictions to the total number of predictions; (2) \textit{Recall} refers to the ratio of correct predictions to the total number of samples in the golden test set; and (3) \textit{F1} is the harmonic mean of precision and recall. 


% When comparing the performances, we care more about F1 since it is balanced for evaluation. Note that the correction XXX.


\subsubsection{Results}

\input{table/distilled-size}

%\input{table/syn-perf} 


%\input{table/sem-perf} 



Table \ref{table:rq2_dataset} demonstrates the performance of our syntactic cleaner in terms of noisy data detection. We can see that, the syntactic cleaner can precisely detect syntactic noises on the four benchmark datasets. The Micro F1 scores are ranging from 93.76\% to 95.5\%, and 94.65\% on average, which is highly satisfactory.
%The accuracy of syntactic noise correction are ranging from 92.06\% to 95.18\%, which is also highly satisfactory. 
Table \ref{table:sem-perf} shows the performance of our semantic cleaner. We can see that, the F1 scores of non-summary classification are ranging from 86.67\% to 92.86\%, and 91.74\% on average. The results show that, the semantic cleaner can also achieve a highly satisfactory performance on filtering non-summary noises.

\noindent
\begin{boxedminipage}[t]{\columnwidth}
\jie{i think it isn't necessary to treat this as a separate finding. this is not a finding. }
\textbf{Finding 1}: Our code-summary cleaner can precisely filter noisy data syntactically and semantically, with all the F1 scores of over 90\%.  
\end{boxedminipage}

==> bak/6.discussion.tex <==
\section{Discussion}
Results from this study suggest several interesting findings that can serve as the practical guidelines for improving code summarization regarding the collection and selection of benchmark data.%\ye{See comment.}
%Ye: the current discussion content appears piece-wise and not cohesive. Suggested reorganization:
%7.1 Common anti-patterns of data preprocessing in code summarization 这一部分最后要呼应、扣本文标题
%7.2 Tool implementation to cope with anti-patterns 这一部分突出工具的接口design、易用性考量，以及开源
%7.3 Guidelines for improving data quality： 这一部分要强调collaborative community effort，从数据预处理的设计和质量监控、以及论文审稿checklist等等方面给出具体操作建议


%数据集质量提升

%\section{Application}
%\subsection{A Data Cleaning Tool}

%\subsection{An Evaluation Hub}

%1 是 收集新数据时候应该注意到地方, 
%suggest preprocessing operation set

%^2 是模型的训练 验证 如何使用已有的数据 做一些建议

%3 extensive application. our tool can also apply to other code-text data for text to code or code to text tasks.

\subsection{On the Importance of Data Quality.}
%\textbf{On the importance of data quality.}
%Data has long been a integral ingredient for learning-based SE tasks. Recently, 
Data quality has been a growing concern, especially since
deep learning (DL) is being widely applied for massive SE tasks. As DL models typically require high-volume data, ensuring data quality at a large scale has become a compelling need. %more challenging. 
Most existing studies focus on advances in modeling but typically overshadowed the quality of data. When investigating the existing code summarization models (as shown in Table \ref{table:dataset_intro}), we notice that a substantial amount of data preprocessing operations are cursory or lack of consistency. % statements. 
%\ye{see comment}. %Ye: "sketchy" --> cursory? "not comprehensively stated" -- > lack of consistency or unconvincing? 
In addition, there is the lack of principles or methods to guide and reinforce the data preprocessing associated effort while conducting code summarization research, regarding how to soundly preprocess benchmark datasets for different tasks.
For instance, our results show that noisy data extensively exist in the four widely-used benchmark datasets for code summarization tasks. Shi \textit{et al.}~\cite{DBLP:journals/corr/abs-2107-07112} reported that different code preprocessing operations can affect the overall performance of code-summarization models by a noticeable margin. 

Therefore, it is recommended to pay more attention to data quality while training code summarization models, rather than directly reusing existing datasets without quality inspection. Based on our \textit{Finding 2}, we argue that the existing models used for code summarization tasks in the literature have a great potential of improvement given a large, good-quality dataset. \ye{see comment.} %Ye: 这一部分的呼吁好像不是很明确，是要进一步阐明问题严重性？是要建议推广采纳类似本文提出的情绪工具？还是改进对论文审稿中加强对数据质量的把关？

%\subsection{Implications}
%\noindent


%However, the data quality is typically overshadowed by advances in modelling. 


%currently lack best practices and principled methods regarding how to efficiently build datasets for different SE tasks



%现在的问题，DL in SE 在data quality的重视不够,列举其他著名领域的数据预处理问题，比如论文里不交代，或者有些明显的错误
%我们深入分析了code summarization,发现影响较大。
%这里我们给出了code-text数据清理的建议：1234
%呼吁：其他的tasks，也应该有类似的工作，可参考我们的methodolody


% \textbf{On the evaluation datasets.}
% %Diversity of evaluation datasets.
% When analyzing the impacts of noisy data on code-summarization model performance, we also notice that, the ranking among the three types of models does not preserve when evaluating them on different datasets. For example, Rencos (IR+NN) outperforms other models in TLC but is worse than NSC (NN) in Funcom and PCSD, as shown in Table \ref{table:rq3_result}. 
% To more comprehensively evaluate different code-summarization models, it is recommended to use multiple datasets, as the ranking of the model can be inconsistent on different datasets.



\subsection{Implications for Data Preprocessing}


%\noindent 
%\textbf{Lessons Learn for building new datasets in code summarization tasks.}
\textbf{Anti-patterns for data preprocessing.}
Based on the results of the quality assessment on benchmark datasets, we discuss the following anti-patterns to avoid when future code summarization researchers build their own datasets. 
\begin{itemize}[leftmargin=4mm]
\item Assuming the first sentences of comments is representative. Rationale: the results show that using first sentences of comments is error-prone. 
\item More comment is better. Rationale: the results show that we should be careful of ``what to comment'', check whether the following types of code-comment data are suitable for your scenarios: interrogative comments, auto code, duplicated code, block-comment code.
\item Over-splitting of variable identifiers in comments. Rationale: ...
\item Including under-development or out-of-date code, e.g., TODOs, commented-out methods. Rationale: ...
\item Remember to deal with abnormality, e.g., HTML tags, URL, code path, non-literal natural languages. \ye{This sentence needs to be converted into the description of an anti-pattern.}
\end{itemize}
%




\textbf{Need for researches on inconsistent code-comment detection.}
In this study, we define 12 categories of noisy data in code summarization datasets, and apply our cleaning tool to filter them out. For the filtered data, there might exist other hidden noises in that comments are not consistent with the code in benchmark datasets, e.g., obsolete comments during software evolution. Based on our manual inspection on the 1,174 code-comment pairs that are annotated as non-noisy comments in section 3, 14 of them are such inconsistent pairs. \ye{See comment.} % 14 inconsistent pairs out of 1174, which might weaken the severity of this inconsistent pair issue. Do you have stronger evidence on the scope or severity of the issue?
The following example shows a spotted inconsistency between the comment and its code. The comment explicitly states the return fact but the code does not.   
Since only a few approaches are proposed for detecting inconsistent Java code-comment pairs  \cite{DBLP:journals/sqj/CorazzaMS18,DBLP:conf/iwpc/RabbiS20}, and there is a lack of inconsistent code-comment detection for other programming languages, such as Python, and C\#, it is quite challenging to assess and clean such noises in a parallel corpus. Therefore, there is a need for researches on comprehensive inconsistent code-comment detection, which can further benefit the quality improvement of code-comment datasets.

\begin{lstlisting}
/* Read information object and return pointer */
public void readInformationObject(...){
  try {objectDecoder.checkResolved(infoObj);
  } catch (  final Exception e) {
    LogWriter.writeLog("Exception: " + e.getMessage());
  ...
 \end{lstlisting}
    \vspace{-2mm}
\begin{small}
\texttt{Comment (TLC): read information object and \textcolor{red}{return pointer}}\\
\texttt{Code (TLC): public \textcolor{red}{void} read information object...}
\end{small}
\vspace{2.5mm}




%\noindent \textbf{Suggestions for code-summarization models (Finding 3)}
%how to select benchmark dataset? 

\textbf{Considerable noise of duplicated code.}
%Code duplication is common in software development practice. This is often because developers copy and paste code snippets and source files from other projects~\cite{DBLP:journals/pacmpl/LopesMMSYZSV17}. 
Despite the debate on the harmfulness of code clone (i.e., duplicated code) in a software project, i.e., on the one hand-code cloning is considered a harmful practice for software maintenance as it requires consistent changes of the entities that share the same cloned fragment~\cite{lozano2007evaluating}, on the other hand, code cloning can often be used in a positive fashion such as maintaining system stability and tracking code ownership~\cite{kapser2008cloning}. 
In this work, we consider duplicated code as noise and can be harmful to code summarization models. First of all, it is inline with the data preprocessing principle of learning-based models, i.e., the training set should not contain samples in the test set. 
%However, ignoring code duplication may 
Second, keeping code duplication can result in model performance and generalizability not being comprehensively evaluated when applied the models to different benchmark datasets that do not share duplicates.\ye{not following the previous sentence.} Therefore, it is considerable to define duplicated code as noisy data. %In this study, to thoroughly understand the inside information of existing benchmark datasets, we consider the duplicate code as noisy data. 
To facilitate other researches that treat them as normal data, we make the duplicate-code rule switchable in our cleaning tool. \ye{See comment.} %Ye: this part is a little distracting...Maybe i didn't get the point.

%这个有点纠结，因为，如果重复是数据集的客观现象，那就不算是问题。如果重复与数据集的客观分布不同，那就是问题。还有就是，从我的角度，我会认为：如何避免overfitting应该是方法本身应该具备的特性。而不是数据集“应该”帮助算法完成的。


%[] =C. V. Lopes, P. Maj, P. Martins, V. Saini, D. Yang, J. Zitny, H. Sajnani, and J. Vitek, “D´ej`avu: a map of code duplicates on github,” in OOPSLA, 2017.
\subsection{Application}\ye{Why "application"? should we rename it to "Tool implementation"?}



%Our automatic cleaning tool can be integrated into IDEs such as Pycharm or IDEA as a 3rd party plugin. The plugin can determine whether the code comments written by developers follow the common practice guidance. For example, when developers write javadoc comments, our model can automatically extract the first sentences of the comments and classify whether the first sentence is summary. If not, a prompt message would be given. Besides, developers can easily extend the plugin by customizing new rules based on domain-specific documentation guidance. 

%It also opens the door for building large pretrained models to jointly learn code and NL representations that can be leveraged in downstream tasks that do not have adequate data, 

%We release a Natural language comments cleaner


%We release cleaners for Java, Python, respectively.

%we release a filtered compound code-comments pair dataset for Java(Deepcom, Funcom，TLC，XXX）Python(), C#()

We release the implementation of our code-comment cleaning tool as a third-party Python library, named Code-comment cleAning Tool (CAT)\cite{cat_pypi}\ye{do we want to move the name of the tool to the early section?}, which can be easily integrated into the development pipeline of any code summarization model. The features of CAT are:
(1) \textbf{Configurable Rules}. The ruleset in CAT is configurable, which allows users to customize the rules based on the different data characteristics. Besides, users can easily extend the machine learning features that we defined in the model-based semantic cleaning tool by designing new features or removing existing features.
(2) \textbf{Support for Multiple Programming Language}. CAT is a language-independent tool that can support multiple programming languages such as java, python, and c#. Similarly, for applying CAT to other programming language datasets, users can replace the existing language-specific rules with the new rules.
We also release the distilled four benchmark datasets on our website~\cite{website} to facilitate future code summarization research. 

In this study, we explore the data quality issues for code summarization exclusively. We believe the problems we found also exist in other tasks on the intersection of Natural Language Processing and Software Engineering, such as {commit message generation~\cite{jiang2017automatically} (generates a natural language summarization for each submitted code change), code search~\cite{gu2016deep} (generates API usage sequences for a given natural language
query), and code synthesis~\cite{wei2019code} (synthesizes code based on natural language intents), etc. \ye{the previous sentence is very long, and seems like a conclusion.}
Similar to code summarization, the above tasks also require datasets that contain a large number of code and natural language description pairs to train their models, the quality of their datasets can have critical impact on the performance of models. Thus, we recommend future research on these topics should also apply CAT to remove potential data preprocessing noises.}
In addition, we believe CAT can also facilitate the downstream tasks with building large pre-trained {code models~\cite{karmakar2021pre} to %jointly learn code and NL 
learn code representations, %such as code refactoring, clone detection, etc., 
which require a large corpus of code. CAT can help remove code noises as listed in Table~\ref{tab:taxonomy}.}

% Besides the four studied benchmark datasets, we apply our tool on x additional public datasets for code summarization tasks: CodeNN, CSN-py, CSN-csharp, CoDesc. Table \ref{table:app-dataset} shows their details.

% \input{table/app-datasets}

%give a table to report dataset, source, language, \#orgin pairs, \#filterd by SYN, \#filterd by SEM .

\subsection{Threats to Validity}
%threat: there still may unfiltered noise, hard to find, e.g., inconsistent code and comments. 

One threat to validity relates to the random sampling process. Sampling may lead to incomplete results, \textit{e.g.}, noise taxonomy, we plan to enlarge the analyzed dataset and inspect whether new types of noises are emerging. Moreover, our heuristic rules for data cleaning are elaborated from the four popular benchmark datasets, covering Java and Python. Although we generally believe all similar code-comment datasets may benefit from our cleaning tool, future studies are needed to focus on datasets with other programming languages. 

The second threat might come from the process of manual annotation and card sorting. We understand that such a process is subject to introducing mistakes. To reduce that threat, we establish a labeling team, and perform multiple rounds of labeling to make sure that all participants achieve conceptual coherence about noisy categories.



The third threat relates to the BLEU that is used to evaluate the performance of code summarization models. Recent researchers have raised concern over the use of BLEU \cite{DBLP:conf/sigsoft/RoyFA21}, warning the community that the way BLEU is used and interpreted can greatly affect its reliability. To mitigate that threat, we also adopt other metrics, i.e., ROUGE, METEOR, and CIDEr when evaluating performance.



Another threat to validity is the replication of each model. To ensure that the experimental results are consistent with their papers, we retrain the models using the source code provided by the authors, and reuse the parameters provided by the authors.  
We compare the performance of our re-trained models with the performance reported in the papers. Their performances are comparable. For example,  the METEOR score of Rencos is 21.1 on {\pcsd} in their paper, and our re-train Rencos model is 20.2. 
%The minor difference is inevitable since we evaluate on the filtered test set while they evaluate on the origin test set.  

%Our heuristic rules for data cleaning are elaborated and trained from the four popular benchmark datasets, covering Java and Python. Although we generally believe all similar code-comment datasets may benefit from our cleaning tool, future studies are needed to focus on datasets with other programming languages. 


% However, the evaluation conclusion on the effectiveness of our cleaning tool should not be affected, which is obtained by comparing the performance changes of the models before and after noise removal, rather than the absolute value of the model performance.





==> bak/taxonomy-1.tex <==
%\textit{For the summary data in the benchmark datasets, we identify the following six categories of syntactical noises:}

%\jie{the title of this section is `syntactic cleaner', but the organization is in terms of the categories of noises, and there are lot of content involving the categories of noises, which i think needs further discussion.}

\textbf{Partial sentence.}
%When collecting the first sentence as the short summary, researchers use `new line' as the unique delimiter. However, developers may write their summaries across multiple lines, in such cases, the `new line' delimiter will lead to the incomplete collection of the first sentences.(what lead to that noise). The incomplete first sentence will make the ground-truth summary shorter and thus easier to generate. (what consequence) Therefore, we use the unfinished-sentence feature, \lin{add e.g., or cite} to identify and update the summary data by adding the missing part back.(our action)
% guide:http://www.oracle.com/technetwork/articles/java/index-137868.html
{Since it is a common practice to place a method's summary at the first sentences of the code comments \cite{technetwork_articles_java}, most researchers use the first sentences of the code comments as the target summaries. We observe that some inappropriate processing will lead to partial first sentences collected by researchers. For example, {\funcom} collect the following comments as ``Returns the high value''.  
As shown in Table \ref{tab:taxonomy}, the benchmark data only extracts the first line as the summary, and the next line that should be part of the first sentence is missing. This is primarily due to automatic splitting using new line character such as ``$\backslash$n''.
%Taking the partial first sentence as the target summary will lose some information, making the ground-truth unable to summarize the overall functionality of the source code. Besides, the partial first sentence will make the ground-truth summary shorter and thus easier to generate. 
%\jie{in this current experimental results, we'd better delete this sentence. }
}


 \begin{lstlisting}
 /*
 * Returns the high-value
 * for an item within a series.
 */
 \end{lstlisting}



\textbf{Verbose sentencee.} 
%When collecting the first sentence as the short summary, researchers use `period' as the unique delimiter. However, developers may write their summaries across multiple lines, 
When collecting the first sentence as the target summary, some inappropriate processing used by researchers will lead to verbose first sentences collected. As the example shown in Table \ref{tab:taxonomy}, the {\pcsd} dataset uses the entire code comments as the summary. 
This is mainly because the usage of `period' as the unique delimiter. 
%Verbose first sentences usually contain too much noise, e.g., argument definition or return type of the code, making the code summarization models hard to train.}



\textbf{Content tampering.} Developers may use HTML tags for documentation auto-generation or URLs for external references in comments. We observe that some inappropriate processing will keep the tags or URL contents together with the comments, thus contaminate the benchmark data with meaningless text, e.g., keeping the ``https://developers.google.com/protocol-buffers/docs/encoding'' as ``https developers google com protocol buffers doc encoding'' in the code summary. 
%This kind of noises will lead to the summaries more longer and more difficult to generate, and thus typically will degrade the performance of automatic code summarization approaches.
%Therefore, we remove the code-summary pairs with content tampering noises. 

\textbf{Over-splitting of variable identifiers.} Code summaries likely contain variable identifiers or API terms when describing code functionality. Splitting code by camelCase or snake\_case is a common operation for code understanding \cite{leclair2019neural,DBLP:conf/iwpc/ShahbaziSF21,DBLP:conf/acl/HasanMIMHHAIS21}. However, we observe that some researchers perform this operation on summaries by splitting the contain variable identifiers or API terms in the code summaries, e.g., split `This method initializes jTextField' into `This method initializes j text field'. We consider such operation will change the original meaning of code summaries. 
%Therefore, we update the code-summary pair by recovering the splitted terms. 

\textbf{Non-Literal.} Developers from different countries may write comments in their first languages, mixing with English language in the comments sometimes. We observe that existing benchmark dataset researches occasionally discard the Non-English text but remain the English text as code summaries, as shown in Table \ref{tab:taxonomy}. Since the remaining summary data are typically incomplete and meaningless, we consider them as noises.



\textbf{Interrogation.}
Based on our observation, some of the summaries in the benchmark dataset are interrogations, e.g., 'Is it a good idea using USERID from ASPNET membership table as a foreign key?'. Such interrogations are mainly used for communication, rather than summarizing functionalities.
%Therefore, we remove such noises.

%Developers seem to use comments to communicate with their collaborators during the code review process. There may be some sparse information about the code functionality, but the quality is hard to control. 


%\textit{For the code data in the benchmark datasets, we identify the following five categories of syntactical noises:}

\textbf{Empty Function.} Developers often take on technical debt to speed software development~\cite{wehaibi2016examining}. It has been widely observed that empty function is a common type of technical debt. However, the code-summary pairs extracted from these empty functions can introduce non-trivial noises, this is because an unimplemented empty function and its summary do not match either syntactically or semantically. 
%We remove the code-summary pairs extracted from empty function for data purification.

\textbf{Commented-out method.} Developers often comment out a whole method for deprecating a specific functionality~\cite{falessi2015five}. We observer that the in the studied code summarization datasets, many commented-out methods are collected as the comments for the sequential methods. 
%We consider these code-summary pairs extracted from commented-out methods as noises and remove them for cleaning data. 

\textbf{Block-comment Code.} {We have observed that some code in the benchmark datasets contain block comments inside their bodies. The blocked comments could be natural-language comments or commented-out code. If collecting these blocked comments as code data, the the original logics of the code are likely to be distorted.}
%commenting out code can also at block level except at method level introduced above. 

%Thus, we also remove the commented-out block code for purifying code-summary pairs. 

\textbf{Auto code.} Developers often use modern IDEs like Eclipse or Visual Studio to generate auxiliary functions such as \textit{getter}, \textit{setter}, \textit{toString}, or \textit{tester} for some predefined variables. 
The comments for these {auto generated methods} are often the same as the names of these methods, which makes the code-summary pairs less informative. 
%We consider the code-summary pairs extracted from auto code as noise and remove them for data cleaning purpose.

\textbf{Duplicated code.} 
Developers often reuse code by copying, pasting and modifying to speed up software development \cite{DBLP:conf/oopsla/Allamanis19, DBLP:conf/icse/SajnaniSSRL16}. Identical code appear both in the training and test sets would make the model learn these cases easily and reduce performance on the ``real'' examples while falsely inflating performance metrics such as BLEU or Rouge. %We remove exact duplicates from benchmark datasets and only keeping one copy of them.}
\lin{Might be arguable to define this as noise. Any idea how can we defense if any reviewers disagree?}

\textbf{Non-summary} refer
to comments that are not suitable for the scenario of automated
code summarization.






==> sec/method.tex <==






This study aims to investigate four research questions:

\textbf{RQ1 (Data Pre-processing \rev{Errors} \ye{Illusions})}: How reliable are data pre-processing operations in code summarization tasks?
\ye{I think errors might be a little too strong. The expected contribution may include a list of top assumptions that researchers frequently made in such studies, and a likelihood of leading to potential mismatch/errors, based on data analysis. We can name these "illusions", and the results can Offer cautious warnings/recommendations to mitigate such illusions.}
\lin{Are the benchmarking data syntactically close to code summaries?}

\textbf{RQ2 (\rev{Low-quality} \ye{State of } data \ye{quality})}: What is the code-comment quality in benchmarking datasets? 
\lin{Are the benchmarking data semantically close to code summaries? or Are the ground-truth summaries really summaries, and what quality they have?}






\begin{figure*}[t]
\centering
%\vspace{-0.3cm}
\includegraphics[width=\textwidth]{fig/overview.pdf}
%\vspace{-2.8cm}
\caption{Overview of research methodology.}
\label{fig:overview}
%\vspace{-0.4cm}
\end{figure*}

This study aims to investigate four research questions:

\textbf{RQ3 (Quality Assessment of Cleaned Data}: What is the quality of the benchmark datasets after filtering syntactic and semantic noises? 



\textbf{RQ4 (\rev{Impact on }Performance \ye{Degradation})}: What is the impact of pre-processing errors and low-quality data on the effectiveness of existing code summarization approaches? 


%\textbf{RQ4 (\rev{Progress Assessment} \ye{Research Roadmap or Evaluation Framework})}: How to differentiate the racing paths for code summarization, and what are the progress that existing approaches have achieved?

%\ye{Progress assessment is neutral. To make RQ4 more positive, we can produce a research roadmap with different paths and future work suggestion, or, we can provide a quality-assurance checklist as evaluation framework for code summarization study.}

\subsection{Methodology Overview}
\label{sec: methodology}

Figure \ref{fig:overview} shows an overview of the research methodology. In this work, we focus on evaluating the data quality of four widely used benchmark datasets, \textit{i.e.}, {\pcsd} ~\cite{barone2017parallel}, {\tlc}~\cite{hu2018summarizing}, {\funcom}~\cite{leclair2019neural}, and {\codenn}~\cite{iyer2016summarizing}. %XXXX.\lin{Update}  

For RQ1, we evaluate the syntactic noises in the provided data from summary level and code level. After discarding the syntactically noisy data, we obtain the SYN-clean datasets. 

For RQ2, we evaluate the semantic noises and the quality of the provided summaries in the SYN-clean datasets by three means: 
(1) We conduct a model-based evaluation to analyze the concentration of actual summaries. The model can predict whether a given sentence is a code summary or not. It is trained on the external  dataset manually labeled by Chen et al. \cite{DBLP:journals/tosem/ChenXHLL21}, and tested on a randomly sampled summaries from the SYN-clean datasets. 
(2) We conduct a human evaluation to analyze the accuracy, conciseness, and adequacy on the randomly sampled summaries. 
(3) We conduct a metric-based evaluation to analyze the readability and coherence of the provided summaries.

For RQ3, we investigate the performance variation of the state-of-the-art code summarization approaches after removing both syntactically and semantically noisy summaries in the training sets. 



\subsection{Analysis Design for RQ1}
According to common practice guidance, e.g., Javadoc guidance \cite{}, 
%http://www.oracle.com/technetwork/articles/java/index-137868.html
the first sentences of the code comments typically describe the code functionalities. 
Therefore, nearly all the existing researches extract the first sentences of the code comments as the target summaries. However, we have a concern that developers may not fully follow the guidance when writing comments. 
Meanwhile, since code comments contain rich information, e.g., URLs for external references and HTML tags for documentation auto-generation, existing researches use various preprocessing operations when constructing the code-summary pairs for the benchmark datasets. We have another concern about how well are these preprocessing operations performed. 
In this work, we define the incorrectly extracted first sentences and inappropriate preprocessing consequences as \textbf{syntactic noises}. 
To address the above concerns, we develop a taxonomy of syntactic noises with a set of heuristic rules that can precisely identify and correct them.

\textbf{Taxonomy of syntactic noises.} To develop a taxonomy of syntactic noises for both code data and summary data, we employ an \textit{open card sort} \cite{DBLP:journals/es/RuggM05} process by involving XXX participants. 
The sorting process is conducted in multiple rounds. In the first round,
all participants label the same sample of benchmark data, with an intensive discussion session to achieve conceptual coherence about noisy categories. The average Cohen’s Kappa is 0.86.
Then, a shared pool of categories is utilized and carefully maintained, and
each participant could select existing categories from and/or add new category names into the shared pool. The sorting process ends when there is no new category added for two consecutive rounds. In total, we conducted XX rounds and labeled XXX pairs of code summary (XXX pairs for each four benchmark datasets). We introduce the taxonomy of syntactic noises and their examples in Table XXX. 
  



\textbf{Heuristic rules.} To automatically identify each category of syntactic noises, we build a set of heuristic rules. The heuristic rules comply with three criteria: (1) Any rule should define a unique and
specific construction category; (2) The rules should limit the preclusion of valid data within an acceptable range; and (3) Any rule is not a subrule of other rules in the set.
We build the heuristic rules based on observing the XX\% of our labeled data, and evaluate on the rest 20\%. The average accuracy is XX. Limited by the space, the details of the heuristic rules can be found on our website \cite{}. 

Note that we focus on syntactic noises on summaries and code separately in RQ1, and leave the fine-grained semantic analysis, such as coherence between code and summary, to RQ2.
%We introduce the taxonomy of syntactic noises , their examples, and identification rules in the following.

%and leave the fine-grained semantic analysis to RQ2

%We introduce the syntax features covered by our ruleset in the following, and the feature examples can be found in Table 1.

%怎么找的分类：card sorting?

%怎么自动检索：正则表达规则
%怎么评价规则:


%Table: Category, description, syntax rule, action, example


\subsection{Analysis Design for RQ2}
\mfw{Code summarization refers to the task of generating concise summaries that describe functionality of the code \cite{}. Directly taking the entire or first sentence of a code comment as the ground-truth summary would introduce noise, since developers write comments with a large variety of different meanings. For example, comments may also be used for other intentions, such as copyright and to-do, instead of describing the core functionalities, thus should not be regard as the code summary semantically. In this section, we define the non-summary comments that do not describe the functionalities of the corresponding code as semantic noises. We first introduce a model-based semantic filter to further remove the semantic noises from the SYN-clean datasets. Then, A human evaluation and metric-based evaluation are conducted to analyze the quality of the cleaned benchmark datasets.}






\subsubsection{Semantic noise analysis }XXX.
%\subsubsection{The model-based Semantic filter}



How do we define Semantic noise, summary and non-summary, refer to existing two papers.


Summary Classifier Construction.

Dataset.

Model.(Feature, GBDT)

Summary Classifier Evaluation.


Filtering non-summaries.


\textbf{Model-based Semantic Filter}
In this work, we employ the Gradient Boosting Decision Tree (GBDT) \cite{} as the semantic filter. GBDT is a widely-used machine learning model, and has been proven to be effective in comment classification in software engineering \cite{}. It is an ensemble model of decision trees, which are trained in sequence, and each base model is added to correct the error produced by its previous tree models. For each step, the samples misclassified by previous models are more likely to be selected as the train data, producing more accurate prediction performance.

To enhance features and improve model performance, we consider three categories of features: textual features, statistical features, and syntactic features. For textual features, after tokenization of the comments, we extract tf-idf \cite{} vector of each word, which could determine the mathematical significance of words in comments. Such a technique is a conventional feature extraction approach for the natural language text analysis in the software engineering literature \cite{}. For statistical features, we extract the number of words, unique words, punctuation and digits. For syntactic features, we determine whether a comment contains keywords such as ``todo", ``deprecate", ``copyright", ``lincense". These features are also used in prior software engineering literature \cite{}.

\textbf{Evaluation Metrics}
We use three commonly-used metrics to evaluate the performance of the semantic filter, \textit{i.e.}, Precision, Recall, and F1. (1) Precision refers to the ratio of the number of correct predictions to the total number of predictions; (2) Recall refers to the ratio of correct predictions to the total number of samples in the golden test set; and (3) F1 is the harmonic mean of precision and recall. When comparing the performances, we care more about F1 since it is balanced for evaluation.

% \textbf{Training and Prediction}

\subsection{Analysis Design for RQ3}
\subsubsection{Human-Based Quality Assessment of Code Summary} 
Most existing benchmark datasets for code summarization task are constructed based on real-world code repositories, such as GitHub. 
Since developers have the freedom to write comments in various ways \cite{DBLP:conf/scam/RaniASBN21}, we have a concern about the quality of code summaries provided by the widely used benchmark datasets. 
Therefore, we further assess the summary contents in the four benchmark datasets that are cleaned by our summary classifier.

%To assess the quality of code summaries, we employ human annotators to assess Accuracy, Conciseness, and Adequacy. 


%Typically, data-driven models in the code summarization task require high-quality data.


Deriving from previous evaluations of code summarization \cite{DBLP:conf/iwpc/McBurneyM14,DBLP:conf/kbse/SridharaHMPV10,DBLP:conf/iwpc/SridharaPV11,DBLP:journals/access/SongSWY19}, the ``quality'' of the code summaries was assessed in terms of accuracy, conciseness, and adequacy by human evaluators.


\begin{itemize}
\item {\textbf{Accuracy}} measures to what extent the summaries reflect the semantics of the relevant code.
\item \textbf{Conciseness} refers to what extent the summaries contain the unnecessary information.
\item \textbf{Adequacy} evaluates how much information the summaries miss with regard to the information contained in code. 
\end{itemize}

We use a five-level Likert scale \cite{chisnall1993questionnaire} to score the three aspects (Strongly Disagree, Disagree, Neutral, Agree, Strongly Agree). 
We randomly sample XXX code-summary pairs from the four benchmark data that are classified as `summary' (XXX for each) as our evaluation target. 
{We recruit XX participants, including XX PhD students, XX master students, XX professional developers and XXX senior researchers, all familiar with the java, python and c\# programming languages. They all have at least three years of software development experience, and four of them have more than ten years of development experience.}\lin{@fangwen update}








\subsubsection{Metric-Based Quality Assessment of Code Summary} 
Besides the three human-based quality assessment, we also evaluate the \textbf{Readability} \cite{DBLP:journals/information/EleyanOE20} and \textbf{Coherence} \cite{DBLP:conf/iwpc/SteidlHJ13}
by using predefined metrics following previous studies.

\textbf{Readability} measures the difficulty of understanding the contents of the summaries.
The Flesch Reading Ease has been used to measure the readability of code summaries \cite{DBLP:journals/information/EleyanOE20}.
The Flesch Reading Ease is calculated with the following formula:
\begin{equation}
    FRE=206.835-0.296S-84.6W
\end{equation}
where $S$ is the average number of words used per sentence, and $W$ is the average number of syllables per word. Higher FRE scores indicate summaries that are easier to read; lower scores indicate summaries that are more difficult to read.



\textbf{Coherence} reflects aspects of how the summary and code relate to each other.
The coherence coefficient has been used to measure coherence between the summary and code \cite{DBLP:conf/iwpc/SteidlHJ13}. 
The coherence coefficient is calculated with the following formula:
\begin{equation}
    c\_coeff=
\end{equation}
Summaries with $c\_coeff = 0$ indicate that the coherence between method name and the summary is not sufficient. They should have additional information to emphasize the relation to the method name or indicate a poor method name.
Summaries with $c\_coeff > 0.5$ are trivial as
they do not contain additional information.

\subsection{Analysis Design for RQ3}



==> sec/metric.tex <==
We evaluate the performance of the three baselines using common metrics including BLEU~\cite{DBLP:conf/acl/PapineniRWZ02}, METEOR~\cite{DBLP:conf/acl/BanerjeeL05}, ROUGE-L~\cite{lin2004rouge}, and CIDEr~\cite{DBLP:conf/cvpr/VedantamZP15}. These metrics are also widely used in machine translation, text summarization, and image captioning.

Given the generated summary $X$ and the ground-truth $Y$, BLEU measures the n-gram precision between $X$ and $Y$ by computing the overlap ratios of $n$-grams and applying brevity penalty on short translation hypotheses. BLEU-1/2/3/4 correspond to the scores of unigram, 2-grams, 3-grams and 4-grams, respectively. The formula to compute BLEU-$N$($N$ = 1, 2, 3, 4) is:
\[BLEU-N = BP\cdot\exp{\sum\limits_{n=1}^N{\omega_n\log{p_n}}}\]
where $p_n$ is the precision score of the $n$-gram matches between candidate and reference sentences. $BP$ is the brevity penalty and $\omega_n$ is the uniform weight $1/N$.

ROUGE-L is widely used in text summarization and provides F-score based on Longest Common Subsequence (LCS). Suppose the lengths of $X$ and $Y$ are $m$ and $n$, then:
\[P_{lcs} = \frac{LCS(X,Y)}{m}, R_{lcs} = \frac{LCS(X,Y)}{n},F_{lcs} = \frac{(1+\beta^2)P_{lcs}R_{lcs}}{R_{lcs}+\beta^2P_{lcs}}\]
where $\beta$ = $P_{lcs}$/$R_{lcs}$ and $F_{lcs}$ is the value of ROUGE-L.

For a pair of sentences to be compared, METEOR creates a word alignment between them and calculates the similarity scores by
\[METEOR=(1-\gamma\cdot{frag}^\beta)\cdot\frac{P\cdot R}{\alpha\cdot P + (1 - \alpha)\cdot R}\]
where $P$ and $R$ are the unigram precision and recall, $frag$ is the fragmentation fraction. $\alpha$, $\beta$ and $\gamma$ are three penalty parameters whose default values are 0.9, 3.0 and 0.5, respectively.

CIDEr is usually used for measuring the quality of image captions, which considers the frequency of $n$-grams in the reference sentences by computing the TF-IDF weighting for each $n$-gram. ${CIDEr}_n$ score for $n$-gram is computed using the average cosine similarity between the candidate sentence and the reference sentences. The final result is calculated by combining the scores for different $n$-grams (up to 4).

==> sec/result.tex <==
\section{Results}
\input{table/RQ1_v2}
\subsection{RQ1: Syntactical Noises Analysis }

\subsubsection{Taxonomy}
Table \ref{tab:taxonomy} exhibits the taxonomy of syntactical noises, and demonstrate some real-world examples. 
For the summary data in the benchmark datasets, we identify the following six categories of syntactical noises:

\textbf{Incomplete first sentence.}
%When collecting the first sentence as the short summary, researchers use `new line' as the unique delimiter. However, developers may write their summaries across multiple lines, in such cases, the `new line' delimiter will lead to the incomplete collection of the first sentences.(what lead to that noise). The incomplete first sentence will make the ground-truth summary shorter and thus easier to generate. (what consequence) Therefore, we use the unfinished-sentence feature, \lin{add e.g., or cite} to identify and update the summary data by adding the missing part back.(our action)
{Most researchers use the first sentences of the code comments as the target summaries. We observe that some inappropriate processing will lead to incomplete first sentences collected by researchers. As shown in Table \ref{tab:taxonomy}, the benchmark data only extracts the first line as the summary, and the next line that should be part of the first sentence is missing. This may be because the researchers directly use `new line' as the delimiter. Taking the incomplete first sentence as the target summary will lose some information, making the ground-truth unable to summarize the overall functionality of the source code. Besides, the incomplete first sentence will make the ground-truth summary shorter and thus easier to generate. }


%\input{table/incomplete_first_sen}




% \begin{lstlisting}
% /*
% * Returns the high-value
% * for an item within a series.
% */
% \end{lstlisting}



\textbf{Excessive first sentence.} 
%When collecting the first sentence as the short summary, researchers use `period' as the unique delimiter. However, developers may write their summaries across multiple lines, 
{When collecting the first sentence as the target summary, some inappropriate processing used by researchers will lead to excessive first sentences collected. As the example shown in Table \ref{tab:taxonomy}, the {\pcsd} dataset uses the entire code comments as the summary. 
This is mainly because the usage of `period' as the unique delimiter. Excessive first sentences usually contain too much noise, \textit{e.g.}, argument definition or return type of the code, making the code summarization models hard to train.}



\textbf{Content tampering.} Developers may use HTML tags for documentation auto-generation or URLs for external references in comments. We observe that some inappropriate processing will keep the tags or URL contents together with the comments, thus contaminate the benchmark data with meaningless text, \textit{e.g.}, keeping the ``https://developers.google.com/protocol-buffers/docs/encoding'' as ``https developers google com protocol buffers doc encoding'' in the code summary. This kind of noises will lead to the summaries more longer and more difficult to generate, and thus typically will degrade the performance of automatic code summarization approaches.
Therefore, we remove the code-summary pairs with content tampering noises. 

\textbf{Unnecessary Splitting.} Code summaries likely contain API terms when describing code functionality. Splitting code by camelCase or snake\_case is a common operation for code understanding \cite{leclair2019neural,DBLP:conf/iwpc/ShahbaziSF21,DBLP:conf/acl/HasanMIMHHAIS21}. However, we observe that some researchers perform this operation on summaries by splitting the API terms in the code summaries, \textit{e.g.}, split `This method initializes jTextField' into `This method initializes j text field'. We consider such operation will change the original meaning of code summaries. Therefore, we update the code-summary pair by recovering the splitted terms. 

\textbf{Non-English.} Developers from different countries may write comments in their first languages, mixing with English language in the comments sometimes. We observe that existing benchmark dataset researches occasionally discard the Non-English text but remain the English text as code summaries, as shown in Table X. Since the remaining summary data are typically incomplete and meaningless, we remove such noises.



\textbf{Interrogation.}
Based on our observation, some of the summaries in the benchmark dataset are interrogations, \textit{e.g.}, 'Is it a good idea using USERID from ASPNET membership table as a foreign key?'. Such interrogations are mainly used for communication, rather than summarizing functionalities. Therefore, we remove such noises.
%Developers seem to use comments to communicate with their collaborators during the code review process. There may be some sparse information about the code functionality, but the quality is hard to control. 


For the code data in the benchmark datasets, we identify the following five categories of syntactical noises:

\textbf{Empty Function.} Developers often take on technical debt to speed software development~\cite{wehaibi2016examining}. It has been widely observed that empty function is a common type of technical debt. However, the code-summary pairs extracted from these empty functions can introduce non-trivial noises, this is because an unimplemented empty function and its summary do not match either syntactically or semantically. We remove the code-summary pairs extracted from empty function for data purification.

\textbf{Commented-out \rev{Code}\add{Method}\song{is this right?}.} Developers often comment out a whole method for deprecating a specific functionality~\cite{falessi2015five}. We observer that the in the studied code summarization datasets, many commented-out methods are collected as the comments for the sequential methods. We consider these code-summary pairs extracted from commented-out methods as noises and remove them for cleaning data. 

\textbf{Commented-out block code.} We have observed that commenting out code can also at block level except at method level introduced above. Thus, we also remove the commented-out block code for purifying code-summary pairs. 

\textbf{Auto/Easy Code.} Developers often use modern IDEs like Eclipse or Visual Studio to generate auxiliary functions such as \textit{getter}, \textit{setter}, \textit{toString} for some predefined variables. The comments for these auto generated methods are often the same as the names of these methods, which makes the code-summary pairs less informative. We consider the code-summary pairs extracted from auto code as noise and remove them for data cleaning purpose.

\textbf{Duplicated code.} 
{Developers often reuse code by copying, pasting and modifying to speed up software development \cite{DBLP:conf/oopsla/Allamanis19, DBLP:conf/icse/SajnaniSSRL16}. Identical code appear both in the training and test sets would make the model learn these cases easily and reduce performance on the ``real'' examples while falsely inflating performance metrics such as BLEU or Rouge. We remove exact duplicates from benchmark datasets and only keeping one copy of them.}


\subsubsection{Frequency and Distribution}


Figure \ref{fig:rq1-pie} shows the frequency of total syntactical noises that we removed or updated from the four benchmark datasets. 
Note that, since one code-summary pair may involve multiple noises, we repeatedly count code-summary pairs that involve multiple noise categories when calculating frequency for each category , and count once for the total frequency. Thus, the sum of individual category percentages are slightly higher than the percentage of total noises.\lin{how to simplify this NOTE description.}
We can see that the frequency of total syntactic noises is range from 33.76\% to 60.53\% among the four benchmark datasets, and the average frequency is 43.77\%. Among them, Funcom is the most noisy dataset with 60\% syntactically noisy code-summary pairs, while PCSD is the least noisy dataset with 33\% syntactically noisy code-summary pairs. In the {\tlc} and {\pcsd} datasets, the updated noises are more frequent than removal noises. The other two datasets ({\funcom} and {\codenn}) have a lower frequency of updated noises, especially the {\codenn} dataset has no updated noise. The reason is that the {\codenn} has only Interrogation and Duplicated Code noise, both of which are removal noise.


%\mfw{We can see that the frequency of total syntactic noises is range from 33.76\% to 60.53\% among the four datasets, and the average frequency is 43.77\%. Funcom is the most noisy dataset with 60\% of code-summary pairs containing syntactic noise, while PCSD is the least noisy dataset with 33\% of code-summary pairs containing syntactic noise. In TLC and PCSD datasets, the updated noise is more frequent than removal noise. The other two datasets (Funcom and CodeNN) have a lower frequency of updated noise, especially the CodeNN dataset has no updated noise. The reason is that the CodeNN has only Interrogation and Duplicated Code noise, both of which are removal noise.}


 \begin{figure}[h]
\centering
 \includegraphics[width=\columnwidth]{fig/rq1-pie.pdf}
 %\vspace{-0.3cm}
 \caption{Percentage of syntactic noise in terms of removal and update.}
 \label{fig:rq1-pie}
 \end{figure}

Figure \ref{fig:rq1-heat} illustrates the distribution of each syntactical noise category on the four benchmark datasets. 
The number on each cell presents the percentage of the syntactical noises in the corresponding benchmark dataset.
We can observe that, the benchmark datasets often contain multiple categories of {\SYNN}s.
{\funcom} contains the most {\SYNN} categories (10), followed by {\pcsd} (7) and {\tlc} (6). {\codenn} contains the least {\SYNN} categories (2).
Specifically, there are two primary syntactical issues with Funcom. First, 34.66\% of the code are auto-generated or easy functions such as \textit{setter}, \textit{getter}, \textit{tester}, and \textit{toString} methods\lin{can we format the code with sth like html tag?}.  
Second, 20.01\% of the summaries are split unnecessarily by camelCase. Indeed, previous researches used to complain similar issues that {\funcom} XXX.\lin{@fangwen} \lin{what to say after this...}
The major syntactical issues for {\tlc} is that,  22.85\% summaries are excessive first sentences, and 18.42\% code are duplicated.
The {\SYNN}s in {\codenn} are concentrated in Interrogation. 38.07\% summaries are questions that are used to communicate with collaborators, rather than summarizing code functionalities.
We consider that this phenomenon is related to the collection resources. The code-summary pairs in {\codenn} are collected from Stack Overflow, which is a question-answer platform for developers, while other benchmark datasets are collected from real-world code repositories.   
The primary syntactical issues with {\pcsd} is that, 15.91\% summaries are the incomplete first sentences. 

%大部分数据集中都是多种类型的噪音并存，Funcom中出现了最多10类，其次，PCSD出现了7类，TLC出现了6类，CODENN最少，出现了2类。
%Funcom 主要的问题有两个，一是包含34%的auto/easy code,这里引用现有论文辅助证明。二是做了必须要的切分。
%TLC的主要问题是First Sentence取多了，以及没有去重code
%CODE-NN的问题集中在问句上，解释是因为SO。
%PCSD的问题主要是FS没有取少了。

%\mfw{The number on each cell presents the percentage of the syntactical noises in the corresponding benchmark dataset. Since different data processing methods used by the four datasets, there are obvious differences in the distribution of the noise categories in each dataset. Funcom dataset has the most (10) syntactical noise categories, of which Auto/Easy Code accounts for the highest portion. It means that Funcom contains a large portion of auto-generated methods as well as setter, getter, tester, and toString methods, which was also observed by previous work \cite{}. CodeNN dataset only has Interrogation and Duplicated Code syntactical noise. This is mainly because the CodeNN is collected from SO. It takes the user queries as the target summaries and the corresponding answers as the source code, resulting in the target summaries of CodeNN containing a lot of questions. Due to a query in SO usually has multiple answers, these answers may contain duplicate code.}

%\mfw{Each row presents the frequency of each syntactical noise category on the four benchmark datasets.}



 \begin{figure}[h]
\centering
 \includegraphics[width=\columnwidth]{fig/rq1-heat.pdf}
 %\vspace{-0.3cm}
 \caption{Heatmap for syntactical noises distribution}
 \label{fig:rq1-heat}
 \end{figure}
 
\textbf{Finding 1}: Syntactical noises are extensively existed in the four widely-used benchmark datasets, ranging from 33.76\% to 60.53\%. The primary syntactical issues with the benchmark datasets are: 34.66\% of the code in {\funcom} are auto-generated or easy functions; 22.85\% summaries in {\tlc} are excessive first sentences; 38.07\% summaries in {\codenn} are interrogative; and 15.91\% summaries in {\pcsd} are the incomplete first sentences.


\subsection{RQ2: Semantic Noises Analysis}
\subsubsection{Summary V.S. Non-summary}

\subsubsection{Quality of Code Summary}

\subsection{RQ3: Impact on SOTA Performance}

==> table/RQ2_feature.tex <==
\begin{table}
\centering
\caption{Features for sumamry classification}
\label{tab:rq2_feature}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|l|} 
\hline
\textbf{Category} &\textbf{Feature} & \textbf{Type} & \multicolumn{1}{c|}{\textbf{Description}}                                                    \\ 
\hline
\multirow{8}{*}{\makecell{Statistical\\ Features}} & TF-IDF           & numerical     & \makecell[l]{Measures how often a word appears in a comment\\ and how common the word is in the corpus.}     \\ 
\cline{2-4}
&Words            & numerical     & \makecell[l]{Measures the length of the comment, using the\\ words as unit size, separated by white spaces}  \\ 
\cline{2-4}
&Unique Words     & numerical     & \makecell[l]{Measures the length of the comment, only unique\\ words are counted}                           \\
\cline{2-4}
&Punctuation      & numerical     & \makecell[l]{Measures the percentage of punctuation in a\\ comment (e.g., ":", "+", "", "@")}                \\
\cline{2-4}
&Digits           & numerical     & Measures the percentage of digits in a comment                                               \\ 
\hline
\multirow{10}{*}{\makecell{Content\\Features}} & Uppercase        & boolean       & \makecell[l]{True if all words in the comment are uppercase,\\ such as "NOT YET DDOCUMENTED"}                \\ 
\cline{2-4}
& Todo             & boolean       & \makecell[l]{True if a comment contains keywords such as\\ "todo","TBD"}                                     \\ 
\cline{2-4}
& Deprecation      & boolean       & \makecell[l]{True if a comment contains keywords such as\\ "deprecate", "not in use"}                        \\ 
\cline{2-4}
& Copyright        & boolean       & \makecell[l]{True if a comment contains keywords such as\\ "copyright", "license" }                          \\ 
\cline{2-4}
& Notice           & boolean       & \makecell[l]{True if the start of the comment contains \\keywords such as "FIXME:", "WARNING:"}              \\ 
\cline{2-4}
& Code Snippet     & boolean       & \makecell[l]{True if a comment contains code snippets or\\ mathematical formulas}                            \\
\hline
\end{tabular}
}
\end{table}

==> table/alg.tex <==

\begin{algorithm*}[htbp]
\caption{xxxxx}
\label{alg:algorithm}
% \textbf{Input}: raw comment \textit{RC}, benchmark comment \textit{BC}\\
% \textbf{Output}: The first sentence of raw comment \textit{FS}\\
% The noise category of the benchmark comment NC 
\begin{algorithmic}[1] 
\Require
raw comment $RC$ and benchmark comment $BC$ 
\Ensure 
The first sentence of raw comment $FS$ and the noise category of the benchmark comment $NC$
\State Initialize $FS$ ← `` ''
\State Define $regex1$ = \verb|'^[\s/*]+'|
\State Define $regex2$ =\begin{verbatim}'([^\n]+?)(((?<!i\.e)(?<!e\.g)(?<!\beg)(?!\bie))\.\s|\.$)'\end{verbatim}
\State Define $regex3$ =\begin{verbatim}'^[A-Z@]|(\(?i\.e\.)|(\(?e\.g\.)|(\(?eg\.)|(\(?ie\.)[\s\S]+'\end{verbatim}
\State Split $RC$ into comment list $L$ using newline character \verb|'\n'|
\For{each $l$ $\in$ $L$}
    \If{$FS$ is not empty}
        \If{$l$.match( $regex3$ ) is not none }
            \State break;
        \EndIf
    \EndIf
    \State $l$ ← $l$.sub($regex1$, \verb|''|)
    \If{$l$.match($regex2$) is not empty}
        \State $FS$ ← $FS$ + $l$.match($regex2$);
        \State break;
    \Else
        \State $FS$ ← $FS$ + $l$
    \EndIf
\EndFor
\If{length($FS$) > length($BC$)}
    \State $NC$ ← \verb|"Partial sentence"|
\ElsIf{length($FS$) < length($BC$)} 
    \State $NC$ ← \verb|"Verbose sentence"|
\Else
     \State $NC$ ← ``normal''
\EndIf
\State \textbf{return} $FS$, $NC$;


\end{algorithmic} 
\end{algorithm*}

==> table/app-datasets.tex <==
\begin{table}[ht]
\caption{Additional Filtered Datasets}
\label{table:app-dataset}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Source} & \textbf{Language} & \textbf{Origin} & \textbf{Filtered by syntactic cleaner} & \textbf{Filtered by semantic cleaner} \\ \hline
CodeNN{[}{]}     & Stack Overflow  & C\#              &    66,015             &        40,375                    &     40,042                                  \\ \hline
CSN-py{[}{]}     &                 &                   &                 &                                        &                                       \\ \hline
CSN-C\#{[}{]} &                 &                   &                 &                                        &                                       \\ \hline
CoDesc{[}{]}     &                 &                   &                 &                                        &                                       \\ \hline
\end{tabular}
}
\end{table}

==> table/feature_and_evaluation.tex <==
\begin{table*}[htbp]
\caption{The syntax feature of the heuristic rules and their evaluation results}
\label{tab:feature_and_evaluation}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|cc|c|c|c|c|c|c|c|c|}
\hline

\multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{Category}}} & 
\multirow{2}{*}{\textbf{Syntax Feature}} &
\multirow{2}{*}{\textbf{Action}} &
\multicolumn{3}{c}{\textbf{Dataset}}&
\multicolumn{3}{|c|}{\textbf{Performance (\%)}}
\\ \cline{5-10}
{}&{}&{}&{}&
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\makecell{\#Annotations(100\%)}\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\makecell{Rule-Build(80\%)}\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}\makecell{Rule-Test (20\%)}\end{tabular}} & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \textbf{F1} \\ \hline \hline

\multicolumn{1}{|c|}{\multirow{14}{*}{\textit{Comment}}} & \makecell{Partial\\ Sentence}     & \makecell{Shorter than the corrected\\ first sentence}          & \makecell{UPDATE: Replace with\\ the corrected\\ first sentence } \\ \cline{2-10} 

 \multicolumn{1}{|c|}{}                         & \makecell{Verbose\\ Sentence}     & \makecell{Longer than the corrected\\ first sentence}                                                       & \makecell{UPDATE: Replace with\\ the corrected\\ first sentence } \\ \cline{2-4} 
 \multicolumn{1}{|c|}{}                         & \makecell{Content\\ Tampering}    & \makecell{HTML tags, Doc tags, \\and URL format}  & \makecell{UPDATE: Clean the tags\\ from comment data}\\ \cline{2-4} 
 \multicolumn{1}{|c|}{}                         & Over-Splitting       &\makecell{Split comments on camel\\ case and underscore}                                   & \makecell{UPDATE: Replace the \\over-splitting variables\\ with the original ones } \\ \cline{2-10} 
 \multicolumn{1}{|c|}{}                         & Non-Literal          & non-ASCII                                                                                 & \makecell{REMOVE} \\ \cline{2-10} 

 \multicolumn{1}{|c|}{}                         & Interrogation        & \makecell{``?'', ``what'', ``how'', etc. }                      & \makecell{REMOVE} \\ \cline{2-4} 
 \multicolumn{1}{|c|}{}                         & Under-Development          & \makecell{``todo'', ``deprecate'',\\ ``copyright'',``FIXME:'', etc.}       & \makecell{REMOVE} \\ \hline \hline
 \multicolumn{1}{|c|}{\multirow{10}{*}{\textit{Code}}}    & \makecell{Empty\\ Function}       & The method body is empty                                                                & \makecell{REMOVE} \\ \cline{2-10} 
 \multicolumn{1}{|c|}{}                         & \makecell{Commented-Out\\ Method} & \makecell{The whole method \\is commented out.}             & \makecell{REMOVE} \\ \cline{2-4} 
 \multicolumn{1}{|c|}{}                         & \makecell{Block-Comment\\ Code}   & \makecell{The method contains the\\ block comment.}                                                                                                         & \makecell{UPDATE: Clean the \\blocked comments\\ from the code body} \\ \cline{2-10} 
 \multicolumn{1}{|c|}{}                         & Auto code            & \makecell{setter, getter, tester, etc.}                                                                           & \makecell{REMOVE} \\ \cline{2-10} 
 \multicolumn{1}{|c|}{}                         & \makecell{Duplicated \\Code}      & Exact Match                                  & \makecell{REMOVE} \\ \hline
 
\end{tabular}
}
\end{table*}

==> table/heat.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[htbp]
\caption{Percentage of noisy data in benchmark datasets.}
\label{tab:heat}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|cc|c|c|c|c|}
\hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{2}{|c|}{\textbf{Category of Noisy Data }}   & \textbf{Funcom }                         & \textbf{TLC }                            & \textbf{CSN }                            & \textbf{PCSD}                         \\ \hline
\multicolumn{1}{|c|}{}                          & Partial Sentence     & \cellcolor[HTML]{D78070}17.1 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{DC8E78}7.8  & \cellcolor[HTML]{D78271}15.9 \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Verbose Sentence     & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{D3776B}22.8 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{DC8E78}7.8  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Content Tampering    & \cellcolor[HTML]{DB8B77}9.7  & \cellcolor[HTML]{DE967C}3.2  & \cellcolor[HTML]{D27469}24.4 & \cellcolor[HTML]{E7B38B}0.5  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Over-Splitting       & \cellcolor[HTML]{D3756A}24.1 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Non-Literal          & \cellcolor[HTML]{E6B28B}0.5  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{DC8E78}7.8  & \cellcolor[HTML]{EDCB97}0.2  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Interrogation        & \cellcolor[HTML]{E2A182}0.7  & \cellcolor[HTML]{DF997E}0.9  & \cellcolor[HTML]{E2A182}0.7  & \cellcolor[HTML]{EABE91}0.3  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Under-Development    & \cellcolor[HTML]{DE957C}3.7  & \cellcolor[HTML]{DF997E}1.2  & \cellcolor[HTML]{DF997E}1.2  & \cellcolor[HTML]{DF977D}2.3  \\ \cline{2-6} 
\multicolumn{1}{|c|}{\multirow{-8}{*}{Comment}} & \textit{Total}       & 40.9                         & 25.4                        & 36.1                         & 26.5                         \\ \hline
\multicolumn{1}{|c|}{}                          & Empty Function       & \cellcolor[HTML]{DF987E}1.6  & \cellcolor[HTML]{DF997E}1.1  & \cellcolor[HTML]{F1D89E}0.0  & \cellcolor[HTML]{F1D99E}0.0  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Commented-Out Method & \cellcolor[HTML]{ECC795}0.2  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Block-Comment Code   & \cellcolor[HTML]{DA8975}11.1 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Auto Code            & \cellcolor[HTML]{CF6B64}29.8 & \cellcolor[HTML]{DD947B}4.6  & \cellcolor[HTML]{DF987E}1.6  & \cellcolor[HTML]{DE947B}4.3  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & Duplicated Code      & \cellcolor[HTML]{E5AE89}0.6  & \cellcolor[HTML]{D67E6F}18.4 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{DF987E}1.5  \\ \cline{2-6} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{Code}}    & \textit{Total}       & 40.7                         & 22.6                         & 1.6                          & 5.8                          \\ \hline \hline
\multicolumn{2}{|c|}{Removed noisy data}                               & 38.7                         & 21.1                         & 29.2                        & 9.3                         \\ \hline
\multicolumn{2}{|c|}{Updated noisy data}                               & 27.1                         & 20.8                         & 8.0                          & 21.9                         \\ \hline
\multicolumn{2}{|c|}{Total}                                            & 65.8                         & 41.9                         & 37.2                         & 31.2                         \\ \hline
\end{tabular}
% \begin{tablenotes}
% \footnotesize
% \item \textbf{$*$} denotes the pull requests receive ``like'', ``great'' or ``nice'' in GitHub.
% \end{tablenotes}
}
\end{table}

==> table/heat_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\caption{Distribution of noisy data in benchmark datasets.}
\vspace{-0.2cm}
\label{tab:heat}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|cc|c|c|c|c|}
\hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{2}{|c|}{\textbf{Category of Noisy Data }}   & \textbf{\funcom}                         & \textbf{\ \ \tlc\ \ \ \ }                            & \textbf{\ \ \codenn\ \ \ \ }                            & \textbf{\ \ \pcsd\ \ \ }                         \\ \hline
\multicolumn{2}{|c|}{\textit{Total}}  &
\hspace{-1.3cm}
\begin{minipage}{}
    \includegraphics[width=1.2cm,height=1.2cm]{fig/pie/pie-1.pdf}
\end{minipage} &
\hspace{-1.3cm}
\begin{minipage}{}
    \includegraphics[width=1.2cm,height=1.2cm]{fig/pie/pie-2.pdf}
\end{minipage}&\hspace{-1.3cm}
\begin{minipage}{}
    \includegraphics[width=1.2cm,height=1.2cm]{fig/pie/pie-3.pdf}
\end{minipage}&\hspace{-1.3cm}
\begin{minipage}{}
    \includegraphics[width=1.2cm,height=1.2cm]{fig/pie/pie-4.pdf}
\end{minipage}&
\hline \hline
\multicolumn{1}{|c|}{\multirow{10}{*}{\textit{Comment}}}                         & \makecell{Partial Sentence}     & \cellcolor[HTML]{D78070}17.1 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{DC8E78}7.8  & \cellcolor[HTML]{D78271}15.9 \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Verbose Sentence}     & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{D3776B}22.8 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{DC8E78}7.8  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Content\\ Tampering}    & \cellcolor[HTML]{DB8B77}9.7  & \cellcolor[HTML]{DE967C}3.2  & \cellcolor[HTML]{D27469}24.4 & \cellcolor[HTML]{E7B38B}0.5  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Over-Splitting}       & \cellcolor[HTML]{D3756A}24.1 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Non-Literal}          & \cellcolor[HTML]{E6B28B}0.5  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{DC8E78}7.8  & \cellcolor[HTML]{EDCB97}0.2  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Interrogation}        & \cellcolor[HTML]{E2A182}0.7  & \cellcolor[HTML]{DF997E}0.9  & \cellcolor[HTML]{E2A182}0.7  & \cellcolor[HTML]{EABE91}0.3  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Under-\\Development}    & \cellcolor[HTML]{DE957C}3.7  & \cellcolor[HTML]{DF997E}1.2  & \cellcolor[HTML]{DF997E}1.2  & \cellcolor[HTML]{DF977D}2.3  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}& \textit{Total}       & 40.9                         & 25.4                        & 36.1                         & 26.5                         \\ \hline \hline 
\multicolumn{1}{|c|}{\multirow{8}{*}{\textit{Code}}}                          & \makecell{Empty Function}       & \cellcolor[HTML]{DF987E}1.6  & \cellcolor[HTML]{DF997E}1.1  & \cellcolor[HTML]{F1D89E}0.0  & \cellcolor[HTML]{F1D99E}0.0  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Commented-Out \\Method} & \cellcolor[HTML]{ECC795}0.2  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Block-Comment\\ Code}   & \cellcolor[HTML]{DA8975}11.1 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{F1D99E}0.0  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Auto Code}            & \cellcolor[HTML]{CF6B64}29.8 & \cellcolor[HTML]{DD947B}4.6  & \cellcolor[HTML]{DF987E}1.6  & \cellcolor[HTML]{DE947B}4.3  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                          & \makecell{Duplicated Code}      & \cellcolor[HTML]{E5AE89}0.6  & \cellcolor[HTML]{D67E6F}18.4 & \cellcolor[HTML]{F1D99E}0.0  & \cellcolor[HTML]{DF987E}1.5  \\ \cline{2-6} 
\multicolumn{1}{|c|}{}    & \textit{Total}       & 40.7                         & 22.6                         & 1.6                          & 5.8                          \\ \hline \hline
\multicolumn{2}{|c|}{\textit{Removed noisy data}}                               & 38.7                         & 21.1                         & 29.2                        & 9.3                         \\ \hline
\multicolumn{2}{|c|}{\textit{Updated noisy data}}                               & 27.1                         & 20.8                         & 8.0                          & 21.9                         \\ \hline
% \multicolumn{2}{|c|}{Total}                                            & 65.8                         & 41.9                         & 37.2                         & 31.2                         \\ \hline
\end{tabular}
% \begin{tablenotes}
% \footnotesize
% \item \textbf{$*$} denotes the pull requests receive ``like'', ``great'' or ``nice'' in GitHub.
% \end{tablenotes}
}
\end{table}



==> tmp/todo.tex <==
TBD

add one baseline - TBD
维护website-fangwen(after submit)

==Checklist===
全文统一数字格式用逗号，e.g., 1600 -> 1,600 
all numbers are correct
1-9用term, 10以上用数字
数值小数点保留2位，百分比1位
Funcom 等数据集顺序,名字字体统一
pre-processing -> preprocessing
benchmarking dataset -> benchmark dataset
observer->observe
全文统一: impact of the performance of code summarization
title or sub title 首字母都大写
et al. e.g. i.e. etc 都斜体
fix  ??, ref to table/fig using XX
-遗留问题，如syntact, semantic
-noises.
-规范BLEU等指标写法全文保持一致
-统一dataset name TLC, CSN
fix format issues, e.g.:tiny fonts
all tab/fig are referred
add tool name CAT
===URGENT====
很多地方用第一人称的说法尽量改成第三人称，比如our cleaning tool， our study等改成the cleaning tool和this study比较客观
把we construct the rules这一类说法改成第三人称的被动时，比较客观,如the heuristic rules are constructed ....
In summary, our code-comment cleaning tool can precisely filter noisy data, with all the F1 scores of over 90.0\%, 这个precisely读起来语气太strong，容易引起reviewer不适，这里改成accurately
===URGENT====









==> tmp/website.tex <==
% website: https://github.com/BuiltOntheRock/FSE22_BuiltOntheRock

% github account: BuiltOntheRock
%        password: FSE22_2022_3_17

% mail address: FSE22_built_on_the_rock@outlook.com
%        password: FSE22_2022_3_17
